ARDA: Automatic Relational Data Augmentation for Machine Learning

Automatic machine learning (\AML) is a family of techniques to automate the process of training predictive models, aiming to both improve performance and make machine learning more accessible. While many recent works have focused on aspects of the machine learning pipeline like model selection, hyperparameter tuning, and feature selection, relatively few works have focused on automatic data augmentation. Automatic data augmentation involves finding new features relevant to the user's predictive task with minimal ``human-in-the-loop'' involvement. We present \system, an end-to-end system that takes as input a dataset and a data repository, and outputs an augmented data set such that training a predictive model on this augmented dataset results in improved performance. Our system has two distinct components: (1) a framework to search and join data with the input data, based on various attributes of the input, and (2) an efficient feature selection algorithm that prunes out noisy or irrelevant features from the resulting join. We perform an extensive empirical evaluation of different system components and benchmark our feature selection algorithm on real-world datasets.

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

% \textcolor{red}{N: Organziation of intro is as follows: 
% \begin{enumerate}
%     \item p1: motivation for a system that augments features given large public datasets, and growing reliance of ML on larger datasets.
%     \item p2: key message- people should spend more time on designing algorithms, we can automate data curation/discovery.
%     \item p3: explicit example for what such a system can do
%     \item p4: first challenge in such a system-inferring relatedness for learning tasks, easy for humans, intractable in general. 
%     \item p5: natural approach of building semantic understanding doesn't apply in this setting, data doesn't come with semantic context
%     \item p6: next natural approach of joining everything doesn't work coz ml models are extremely brittle to noise
%     \item p7: we describe what actually works. 
% \end{enumerate}
% }

Today we have the access to tremendous amounts of data on the web. Google Dataset Search 
provides a simple interface to mine data from various sources. Governments, academic 
institutions and companies are making their data sets publicly available. This, combined with
the astonishingly increasing use of machine learning (ML) in data driven
applications has led to a growing interest in integrating ML and data curation/processing. However, existing ML toolkits and frameworks assume that the data is stored in a single table on a single machine. On the contrary, most of the data is stored across the web, in an unstructured form across multiple tables connected by key-foreign key dependencies (KFKDs). 

Since the success of modern ML techniques, such as Deep Learning, is contingent on larger training sets and more features, 
%and data is spread across multiple heterogeneous sources, 
analysts spend a majority of their time finding relevant data to answer the questions at hand, instead of trying various algorithmic solutions and analyzing the results. 
The need for data and feature discovery has therefore opened the door for a new research area that tries to utilize this additional features for improving prediction tasks. Data Enrichment is one such area that only recently defined itself as a response to a need of improved ML predictions by agglomerating data from external knowledge sources. This paper focuses on the problem of Data Augmentation, a pre-processing step that supplements the base data for a ML task by finding and adding relevant features from multiple heterogeneous sources.  
%information derived from internal and external sources within an enterprise. Large publicly available data sets combined with the success of ML techniques have opened the door for a new research area that tries to utilize even more data for improving prediction tasks.  


For instance, consider the critical task of predicting the taxi demand for a given day. Accurate prediction is important for taxi companies in order to dispatch the right amount of cars for cost optimization. The company gathers the history of all the taxi trips over a period of time, as well as statistics of the trip like start time, end time, distance covered, route taken and so on. However, given information might not be enough for accurate predictions of the future demand, even for the "perfect" learning model. In this scenario the remaining solution is to search for external knowledge that we can augment in original dataset to improve the prediction. An example of such knowledge source is a weather dataset that is implicitly connected with taxi data through a key-foreign-key (KFKD) relationship on time series columns. Weather datasets are readily available online and can be successfully incorporated using the join procedure. 

While in this example it wasn't hard for us to infer the strong correlation between taxi demand and weather conditions, automating such inference for different tasks over massive, unstructured data is extremely challenging.
Knowledge Discovery and Data Mining study algorithms to extract a 
semantic understanding from large amounts of unstructured data. However, for a given 
predictive task, the space of possible augmentations grows exponentially in the size of the 
data and a semantic understanding does not provide new features to augment our initial 
dataset. Exploring each possibility quickly becomes computationally infeasible. 
%Further, each augmentation adds a computational overhead in terms of data cleaning, pre-processing and 
performing a join. 
%Hence, there is a need for a system that automatically and efficiently 
%discovers relevant features to extract from a large space of potentially joinable tables, 
%such that the features improve the performance of the prediction algorithm.

Since most of the open source datasets have only meager unstructured description, or no description at all, we cannot rely on semantic relationships between datasets to infer their logical connections. 
%It is also possible that semantic relationships do not imply feature-target correlation. 
For example, taxi and weather has small semantic correlation, but very strong predictive correlation for the aforementioned learning task. Therefore, apriori, we do not know what features are useful in the prediction task and what features are coming from spurious irrelevant datasets. 

Further, agnostically adding all joinable features at once results in an extremely noisy training set. Existing ML models are brittle to noise and thus generalize poorly in such a setting. In particular, massive noise can wash out existing signal and prediction performance may drop below the baseline score altogether. Traditional feature engineering approaches applied to such a training set do not perform well since most of the data may not be correlated with the prediction task at hand as most of the signal has been washed away. 
%indicating that there is no augmentation features present in given sources, while in reality the model is tripped by spurious relations. 
Therefore, we require a system that automatically and efficiently 
discovers relevant features to extract from a large set of potentially joinable tables, such that the augmented data set improves the generalization error of the ML model.  

Our main contribution is to design an end-to-end system that receives as input a prediction task, labelled data, and access to a large repository of unstructured data and augments the initial dataset with new features from the repository, to obtain better performance on the prediction task. The input to our system  includes labelled data in the form of a base table and access to a large database of raw, unlabelled data. After cleaning up the data, we compute a set of joinable tables based on KFKD dependencies. Given this large search space, we integrate the joining procedure with a novel feature selection algorithm that filters out data uncorrelated with the prediction task. 



Our system makes no assumptions about the unstructured data available or about the prediction task and thus provides a universal solution. Since our system is highly modular, users can customize the feature selection, joining approach, coreset construction, and estimators based on specialized tasks at hand. Additionally, our system introduces a noise injection based selection algorithm that may be of independent interest.

We evaluate our system with respect to the prediction performance on the labelled dataset (base table) provided as input, with no augmentation. We benchmark various feature selection algorithms against the one we introduce, where the metric is improvement in accuracy over the base table.



